Unreal-MAP: Unreal-Engine-Based General Platform for Multi-Agent Reinforcement Learning

In this paper, we propose Unreal Multi-Agent Playground (Unreal-MAP), an MARL general platform based on the Unreal-Engine (UE). Unreal-MAP allows users to freely create multi-agent tasks using the vast visual and physical resources available in the UE community, and deploy state-of-the-art (SOTA) MARL algorithms within them. Unreal-MAP is user-friendly in terms of deployment, modification, and visualization, and all its components are open-source. We also develop an experimental framework compatible with algorithms ranging from rule-based to learning-based provided by third-party frameworks. Lastly, we deploy several SOTA algorithms in example tasks developed via Unreal-MAP, and conduct corresponding experimental analyses. We believe Unreal-MAP can play an important role in the MARL field by closely integrating existing algorithms with user-customized tasks, thus advancing the field of MARL.

==> MainTex/01-abs.tex <==

% This paper proposes UnrealEngine-based Multiagent Playground (UMAP), 
% a new open-source simulation platform designed for Multiagent Reinforcement Learning (MARL) studies, 
% to investigate the strength and limitations of existing MARL algorithms.
% In recent years, MARL has become a high-value research topic that has attracted great interest.
% However,
% multiagent cooperation is a large concept with a variety of tasks with distinct feature.
% Many state-of-the-art MARL algorithms with excellent performance in one type of problems
% sometimes suffer from declined performance in other problems that differs in the number of agents,
% the goal, the reward, the action space, etc.  
% This suggests that we have not yet found a perfect MARL algorithm for all cooperative scenarios.
% Therefore, it is important that we develop a method to diagnosis, assess and benchmark 
% the advantages and limitations of existing MARL algorithms.
% However, there is an absence of a benchmark design platform
% that not only is able to design sophisticated task environments in 3D world,
% but also provide easy ways to modify, extend and improve existing environments.
% In this paper, we use UMAP framework to design a group of standard diagnosic tasks XXXX
% and evaluate a wide range of algorithms from following perspectives: xx,xx,xx,xx,xx,xx.
% We first highlight following characteristics of UMAP platform:
% (1) easy to design, program, modify, visualize. 
% (2) optimized for large-scale agent cooperation, with off-the-screen (server) acceleration capability.
% (3) On the basis of ensuring experiment repeatability, compatible with most of native UnrealEngine tools.
% Then in experiment section we use XXXX to evaluate the commonly used MARL algorithms,
% and give suggestions about how to select suitable algorithm considering the feature of a given task.

This paper proposes the Unreal-Engine-based Multiagent Playground (Unreal-MAP), 
a new open-source simulation platform designed for Multiagent Reinforcement Learning (MARL) studies, 
to investigate the strengths and limitations of existing MARL algorithms. 
In recent years, MARL has become a high-priority research topic that has attracted significant interest. 
However, multiagent cooperation is a broad concept with various tasks that have distinct features. 
Many state-of-the-art MARL algorithms with excellent performance on one type of problems 
sometimes suffer from a decline in performance when applied to other problems 
that differ in the number of agents, the goal, the reward, the action space, etc. 
This suggests that we have not yet developed a perfect MARL algorithm for all cooperative scenarios. 
Therefore, it is important to develop a method to diagnose, assess, 
and benchmark the strengths and limitations of existing MARL algorithms. 
However, there is an absence of a benchmark design platform 
that can design sophisticated task environments in a 3D world 
while also providing easy ways to modify, extend, and improve existing environments. 
In this paper, we use the Unreal-MAP framework to design a group of standard diagnostic tasks (XXXX) 
and evaluate a wide range of algorithms from the following perspectives: xx, xx, xx, xx, xx, xx. 
We first highlight the following characteristics of the Unreal-MAP platform: 
(1) easy to design, program, modify, and visualize. 
(2) Optimized for large-scale agent cooperation, with off-the-screen (server) acceleration capability. 
(3) On the basis of ensuring experiment repeatability, compatible with most native Unreal Engine tools. 
In the experiment section, we use XXXX to evaluate commonly used MARL algorithms, 
and give suggestions on how to select a suitable algorithm considering the features of a given task.



